Dense image registration and deformable surface reconstruction in presence of occlusions and minimal texture

Deformable surface tracking from monocular images is well-known to be under-constrained. Occlusions often make the task even more challenging, and can result in failure if the surface is not sufficiently textured. In this work, we explicitly address the problem of 3D reconstruction of poorly textured, occluded surfaces, proposing a framework based on a template-matching approach that scales dense robust features by a relevancy score. Our approach is extensively compared to current methods employing both local feature matching and dense template alignment. We test on standard datasets as well as on a new dataset (that will be made publicly available) of a sparsely textured, occluded surface. Our framework achieves state-of-the-art results for both well and poorly textured, occluded surfaces.

==> rotation.tex <==

\subsection{Rotation Handling}

The original gradient-based descriptors are not rotation invariant therefore
break down when tracking a rotating deformable object. We propose a modification
of these descriptors that can be used in the presence of rotation while still
maintaining their robust convergence properties. Original gradient-based
descriptors of a pixel are computed in the global image coordinates. When the
surface is deformed or rotated, its descriptors also change. To be able to track
a rotating surface, the descriptors of a pixel must be somewhat rotation
invariant, and thus must be computed in its local image patch coordinates. If the
surface is rotated, the local image patch coordinates of a pixel must be rotated
accordingly. In the tracking context, the surface shape in the current image is
very similar to the one in the previous image. Therefore, we can use the
reconstruction in the previous frame to correct the orientation for pixel local
image patch coordinates. Each pixel on the template is associated with its
corresponding mesh facet. When the facet changes its orientation, the local
coordinates of pixel is rotated with the same angle. We compute descriptors of
input image pixels in the global image coordinates, the descriptors for template
image pixels will be rotated with the angle as the change in the orientation of
its corresponding facet. We experimentally show that our proposed method is able
to track a rotating deformable object.


==> rotation_results.tex <==
\subsection{Tracking a Rotating Object}  \label{rotation_results}

To demonstrate that the proposed rotation handling technique can track a
rotating deformable object, we ran our tracking algorithm with and without
rotation handling on the well-textured paper dataset with images
rotated 5 degree every frame. This rotation in addition to original surface
deformations introduce large frame-to-frame motions.
Fig.~\ref{fig:rotation_handling} shows that without rotation handling, the original gradient-based descriptors can only track up to 50 degrees of rotation, while the proposed rotation handling technique can track the whole sequence including a full 360 degrees of rotation.

\begin{figure*}[t]
\centering
\newcommand{\figureWidth}{2.1cm}
\begin{tabular}{cccccccc}
\includegraphics[width=\figureWidth]{fig/handle_rotation/without/frame_149} & 
\includegraphics[width=\figureWidth]{fig/handle_rotation/without/frame_151} & 
\includegraphics[width=\figureWidth]{fig/handle_rotation/without/frame_153} & 
\includegraphics[width=\figureWidth]{fig/handle_rotation/without/frame_156} &
\includegraphics[width=\figureWidth]{fig/handle_rotation/without/frame_159} &
\includegraphics[width=\figureWidth]{fig/handle_rotation/without/frame_161} & 
\includegraphics[width=\figureWidth]{fig/handle_rotation/without/frame_167} \\

\includegraphics[width=\figureWidth]{fig/handle_rotation/with/frame_149} & 
\includegraphics[width=\figureWidth]{fig/handle_rotation/with/frame_156} &
\includegraphics[width=\figureWidth]{fig/handle_rotation/with/frame_163} & 
\includegraphics[width=\figureWidth]{fig/handle_rotation/with/frame_175} & 
\includegraphics[width=\figureWidth]{fig/handle_rotation/with/frame_115} & 
\includegraphics[width=\figureWidth]{fig/handle_rotation/with/frame_125} & 
\includegraphics[width=\figureWidth]{fig/handle_rotation/with/frame_141}

\end{tabular}
\caption{Tracking a rotating deformable surface. {\bf Top row:} Without rotation
handling, tracking with the original gradient-based descriptors eventually breaks down. {\bf Bottom row:} The proposed rotation handling technique can track the whole sequence with up to 360 degrees of rotation.}
\label{fig:rotation_handling}
\end{figure*}




==> selfocclusion.tex <==
%\subsection{Self Occlusions}

\draft{
Our tracking framework can be further extended to handle self-occlusions by
incorporating a z-buffer. Based on the reconstruction from the previous frame or
a motion model, self-occluded template pixels can be detected and excluded from
the image energy computation. We used a z-buffer to densely register images of
the self-occlusion dataset in \cite{GayBellile10} and reconstruct the surface in
the presence of large self-occlusions. The qualitative results are provided in
Fig.~\ref{fig:selfocclusion}. With no additional modifications, our method can
reliably predict the shape of the surface in the areas of self-occlusion.

\begin{figure} 
\centering
  \includegraphics[height=3.6cm]{fig/selfocclusion/frame_120.pdf}  \hfill
  \includegraphics[height=3.6cm]{fig/selfocclusion/view.png}  
  \caption{A z-buffer is incorporated into our method to handle self-occlusions. Left: Image registration is still successful in presence of 50\% self-occlusions. Right: the recovered 3D surface shape.} 
  \label{fig:selfocclusion}
\end{figure}

}
